Visual-Inertial Localization for Skid-Steering Robots with Kinematic Constraints

While visual localization or SLAM has witnessed great progress in past decades, when deploying it on a mobile robot in practice, few works have explicitly considered the kinematic (or dynamic) constraints of the real robotic system when designing state estimators. To promote the practical deployment of current state-of-the-art visual-inertial localization algorithms, in this work we propose a low-cost kinematics-constrained localization system particularly for a skid-steering mobile robot. In particular, we derive in a principle way the robot's kinematic constraints based on the instantaneous centers of rotation (ICR) model and integrate them in a tightly-coupled manner into the sliding-window bundle adjustment (BA)-based visual-inertial estimator. Because the ICR model parameters are time-varying due to, for example, track-to-terrain interaction and terrain roughness, we estimate these kinematic parameters online along with the navigation state. To this end, we perform in-depth the observability analysis and identify motion conditions under which the state/parameter estimation is viable. The proposed kinematics-constrained visual-inertial localization system has been validated extensively in different terrain scenarios.

==> tex/notation.tex <==
\section{Notations}
In this paper, we consider a robotic platform navigating with respect the a global reference frame, $\mathcal{G}$. The platform is equipped with a camera, an IMU, and wheel odometers, whose frames are denoted by $\mathcal{C}$, $\mathcal{I}$, $\mathcal{O}$ respectively. To present transformation, we use $^{\mathbf A}\mathbf p_{\mathbf B}$ and 
$^{\mathbf A}_{\mathbf B} \mathbf R$ to denote position and rotation of frame $\mathcal{B}$ with respect to $\mathcal{A}$.
Finally, we use $\breve{\mathbf a}$ and $\delta \mathbf a$ to represent the estimated value and errors in variable $\mathbf a$.
